Vagueness in Predicates and Objects

Classical semantics assumes that one can model reference, predication and quantification with respect to a fixed domain of precise referent objects. Non-logical terms and quantification are then interpreted directly in terms of elements and subsets of this domain. We explore ways to generalise this classical picture of precise predicates and objects to account for variability of meaning due to factors such as vagueness, context and diversity of definitions or opinions. Both names and predicative expressions can be given either multiple semantic referents or be associated with semantic referents that incorporate some model of variability. We present a semantic framework, Variable Reference Semantics, that can accommodate several modes of variability in relation to both predicates and objects.

==> FMDK-source/FMKD-2022-content.tex <==
%-*- mode: LaTeX; root-file: "/localhome/csc5bb/BBcloud/WORK/Research/MyPapers/2022-JOWO/FMKD-2022-plain.tex"; -*-


%\subsubsection*{CONTENT: 18:33}

\def\excludegraphics#1{includegraphics:#1}

\long\def\skipover#1{}

%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}
Classical semantics assumes that one can model reference, predication and quantification with respect to a fixed domain of possible referent objects. Non-logical terms and quantification are then interpreted in relation to this domain: constant names denote unique elements of the domain, predicates are associated with subsets of the domain and quantifiers ranging over all elements of the domain. The current paper explores the wide variety of different ways in which this classical picture of precisely referring terms can be generalised to account for variability of meaning due to factors such as vagueness, context and diversity of definitions or opinions.
Both predicative expressions and names can be given either multiple semantic referents or be associated with semantic referents that have some structure associated with variability. 
A semantic framework \textit{Variable Reference Semantics\/} (VRS) will be presented that can accommodate several different modes of variability that may occur either separately or in combination.
Following this general analysis of semantic variability, the phenomenon of \emph{co-predication\/} will be considered. It will be found that this phenomenon is still problematic, even within the very flexible VRS framework.


%This involves a type of variability that is challenging to account for within a semantic framework even using the very flexible VRS. The nature of the problem will be explored and several approaches proposed in the literature will be evaluated. Finally, a new approach to modelling co-predication is presented, which using VRS but also requires explicit modelling of the
%different ontological categories and individuation criteria associated with different senses of polysemous terms, as well as  specification of relationships between entities of different ontological types that correspond to these different senses. 
\end{abstract}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\begin{keywords}
  Vagueness, Polysemy, Predication, Quantification, Copredication
\end{keywords}

%%
%% This command processes the author and affiliation and title
%% information and builds the first part of the formatted document.
\maketitle






\section{Introduction}
The  notion  of  reference  and  the  operations  of  predication  and
quantification are  fundamental to  classical first-order  logic.  The
standard semantics for  this logic assumes a fixed  domain of possible
referent objects,  with naming constants referring  to unique elements
of the  domain, predicates being  associated to subsets of  the domain
and quantifiers ranging over all the elements of the domain.  Thus, if
$\mathcal{D}$ is the domain of objects that can be referred to, then a
constant name, say  $\pr{c}$, will donate an object  $\delta(\pr{c})$, such that
$\delta(c)\in\mathcal{D}$, and a predicate $P$ will be taken to denote
a  set of  objects  $\delta(P)$, with  $\delta(P)\subseteq\mathcal{D}$.
Then one  can straightforwardly  interpret the  predicating expression
$P(\pr{c})$   as   a   proposition   that   is  true   if   and   only   if
$\delta(\pr{c})\in\delta(P)$.

But  what  if we  are  dealing  with a  language  that  is subject  to
variability  in the  interpretation of  its  symbols: a  name may  not
always refer  to a  unique, precisely  demarcated entity;  a predicate
need not always  correspond to a specific set  of entities. Accounting
for such  semantic variability  requires some generalisation  or other
modification of the classical denotational semantics.

The aim  of the current  paper is not to  propose a single  theory but
rather to  explore some representational possibilities.   In the first
part of this paper I consider different ways in which semantics can be
given to predication in the presence of semantic variability.  I shall
first  consider  some  general  ideas  regarding  different  views  of
vagueness,  in particular  the  \emph{de re\/}  and \emph{de  dicto\/}
accounts of  this phenomenon. I shall  suggest that these need  not be
mutually  exclusive,  but could  be  describing  different aspects  of
semantic  variability.   I  explore  possible  models  of  denotation,
predication and  quantification in  the presence of  such variability,
first informally, with the aid of some diagrams and then in terms of a
formal framework,  based on \emph{standpoint semantics\/} \cite{Bennett11lomorevi,gomez2018dealing,alvarez2022standpoint},  within which
variable  references can  be modelled.   In the  final section  of the
paper I shall consider the problem of \emph{co-predication}.  This has
been  the subject  of considerable  debate in  recent years  and is  a
phenomenon that  throws up  many examples  that pose  difficulties for
different approaches and has been used to try to support/reject models
of semantic variability.



\subsection{Types of Vagueness}


The literature on vagueness has generally assumed that
the phenomena of vagueness could arise from three potential sources
(see e.g.\ \citet{Barnes10a}):

\begin{enumerate}[itemsep=0ex]
\item indeterminacy of representation (linguistic a.k.a\ \emph{de dicto\/}
  vagueness),
\item indeterminacy of things in the world (\emph{ontic\/} a.k.a.\ \emph{de
  re\/} vagueness),
\item limitations of knowledge (\emph{epistemic\/} vagueness).
\end{enumerate}

The   epistemic  view   of   vagueness  has   some  strong   advocates
\citep{Williamson92vague+ig,Williamson94vague,Sorensen2001-SORVAC} and
many  other  take  the  view  that  the  logic  of  multiple  possible
interpretations takes a similar form to logics of knowledge and belief
(e.g.\      \citet{Lawry08approp,Lawry2009aij}).      Indeed,      the
\emph{standpoint  semantics},  which will  be  used  in our  following
analysis can be regarded as being of this form.  However, the question
of whether this is a deep or superficial similarity is not relevant to
our current  concerns; and  the distinction between  \emph{de dicto\/}
and \emph{de  re\/} aspects  of multiple  reference, would  also arise
within an  epistemic account.  So  in the  current paper we  shall not
further consider the epistemic view.


\subsection{\emph{De Dicto\/} Vagueness}

% As I noted at the beginning of this piece, it is generally agreed that
% a major source of vagueness is imprecision of linguistic representations.
% Where people disagree is on whether there may be other, non-linguistic
% sources of vagueness.

A  widely held  view is  that  all vagueness  is essentially  \emph{de
  dicto},  and that  any kind  of vagueness  that seems  to  come from
another source  can actually be  explained in \emph{de  dicto\/} terms
\citep{Lewis86pluralityOfWorlds,Varzi01a}.  A  fairly typical version
of such  an attitude is that of  Varzi who (focusing on  the domain of
geography,  within  which  vagueness  is  pervasive)  takes  a  strong
position against  ontic vagueness.   Varzi's view of  the relationship
between vague terms and their referents is summarised in the following
quotation:
\begin{quote}
``[To]  say that  the referent  of a  geographic term  is  not sharply
  demarcated is to say that the term vaguely designates an object, not
  that it designates a vague object.'' \citep{Varzi01a} 
\end{quote}



Advocates of exclusively  \emph{de dicto\/} vagueness typically favour
some  variety  of  \emph{supervaluationist\/}  account  of  linguistic
vagueness, within which  the meanings of vague terms  are explained in
terms  of a collection  (a set  or some  more structured  ensemble) of
possible       precise       interpretations       (often       called
\emph{precisifications}).   An early  proposal that  vagueness  can be
analysed  in terms  of multiple  precise senses  was made  by Mehlberg
\shortcite{Mehlberg58a},   and   a  formal   semantics   based  on   a
multiplicity  of classical  interpretations was  used by  van Fraassen
\shortcite{Fraassen69a}  to  explain  `the logic  of  presupposition'.
This kind of formal model  was subsequently applied to the analysis of
vagueness by Fine \shortcite{Fine75a},  and thereafter has been one of
the more popular  approaches to the semantics of  vagueness adopted by
philosophers  and  logicians,  and  a somewhat  similar  approach  was
proposed by \citet{Kamp75a}, which  has been highly influential among
linguists.

What one might  call \emph{absolutist\/} versions of supervaluationism
are   those   that,   following   Fine,   hold  to   a   doctrine   of
\emph{super-truth}.\footnote{What       I       call      `absolutist'
  supervaluationism  is what \citet{Williamson03vague+real}  refers to
  as  `traditional' supervaluationism.}   This is  the tenet  that the
truth of  an assertion containing vague terminology  should be equated
with   it   being    true   according   to   all   \emph{admissible\/}
precisifications    \citep{Fine75a,Keefe2000a,Keefe2008a}.    In   such
theories the set of  admissible precisifications is generally taken as
primitive, just as  is the set of possible  worlds in Kripke semantics
for modal logics.  Other,  supervaluation inspired, theories propose a
similar  semantics  based  on the  idea  that  the  truth of  a  vague
assertion  can only  be  evaluated relative  to  a locally  determined
precisification (or set of precisifications), but reject the idea that
the notion  of super-truth  is useful.  One  might call  such theories
\emph{relativist\/}  supervaluation theories.   Such  theories include
that of  \citet{Shapiro06a} and my  own 
{\emph{standpoint semantics\/}
\cite{Bennett11lomorevi,gomez2018dealing}.\footnote{According      to      standpoint
  semantics,  vague  statements  are  true  or  false  relative  to  a
  \emph{standpoint}.  My  notion of standpoint  is formally identified
  with a set  of precisifications determined by a  set of (consistent)
  judgements that are accepted as  true in a given context.  This idea
  is similar to that presented by \citet{Lewis79a}, and elaborated by
  \cite{Gottschling04a}.}
}

% {...\footnote{A couple of sentences describing one of the Author's 
% previous published works have been removed here to maintain anonymity. 
% The description also relates the Author's theory to ideas of
% \citet{Lewis79a} and \cite{Gottschling04a}}}
%%   
% The  semantics   I  shall  present  below
% (Section~\ref{SEC:formal-semantics})  is broadly  supervaluationist in
% style but neutral  as to whether an absolutist  or relativist position
% is taken regarding the appropriate notion of truth.

Apart  from providing a  general framework  for specifying  a \emph{de
  dicto\/} semantics of vagueness,  the supervaluationist idea is also
attractive   in  that   it   can  account   for   
\emph{penumbral connection\/}  \citep{Fine75a}, which many  believe to
be an essential ingredient of an adequate theory of vagueness. This is
the  phenomenon  whereby  logical  laws  (such  as  the  principle  of
non-contradiction)   and   semantic   constraints  (such   as   mutual
exclusiveness  of two  properties ---  e.g. `...  is red'  and  `.. is
orange') are maintained even  for statements involving vague concepts.
The solution,  in a nutshell, being  that, even though  words may have
multiple different interpretations, each admissible precisification of
a language makes  precise all vocabulary in a  way that ensures mutual
coherence of  the interpretation of distinct  but semantically related
terms.


\skipover{
With regard to  the concerns of the current paper,  it is worth noting
that  supervaluationist  accounts  tend  to work  most  smoothly  when
applied to vague predicates, and  face some problems in accounting for
vagueness  that  appears to  reside  within  nominal expressions  (see
e.g.\ \citet{Weatherson03a}).   Later (in Section~\ref{SEC:dedicto}),
I  shall consider  various  possibilities for  recasting vagueness  in
objects as vagueness in predicates. However, I shall argue that such a
reduction  cannot fully  account  for our  intuitive understanding  of
certain  sentences where  a  `vague object'  is  referred to  multiple
times. In order to represent  the meanings of such sentences I propose
a semantics in which  indeterminacy affects the interpretation of both
predicative and nominal expressions.
}



\subsection{\emph{De Re\/} Vagueness}

In natural language, objects are often described as vague. We commonly
encounter sentences  such as: `The smoke  formed a vague  patch on the
horizon'; `The vaccine injection left a vague mark on my arm'; `He saw
the vague  outline of a  building through the  fog'.  In this  kind of
usage,  `vague' means  something like  `indefinite in  shape,  form or
extension'.  Of course, `indefinite' is almost synonymous with `vague'
so this definition is far from fully explanatory.  However, if we take
sentences like  the aforegoing  examples at face  value, they  seem to
indicate that vagueness can be  associated with an object in virtue of
some characteristic of its spatial  extension. One may then argue that
spatial extension is an intrinsic  property of an object, and that, if
an object has a vague intrinsic property, this indicates vagueness `of
the  thing'.   Such  vagueness  may   be  called  \emph{de   re\/}  or
\emph{ontic}.

The  idea  that vagueness  of  objects  is  primarily associated  with
vagueness of \emph{spatial extension\/} has been endorsed and examined
by \citet{Tye90vague-objects}, who  gives the following criterion for
identifying vague objects: ``A concrete object $o$ is  vague if and
only if: $o$ has borderline spatio-temporal parts;
and there is no determinate fact of the matter about whether there
are objects that are neither parts, borderline parts, nor non-parts
of $o$.'' (The second, rather complex condition concerns the intuition
that we cannot definitely identify borderline parts of a vague object. 
The current paper will not consider this second-order aspect of
vagueness.)

\subsection{Combining \emph{De Re\/} and \emph{De Dicto\/} and the Idea
of \emph{De Sensu\/}}

Rejecting the possibility of  \emph{de re\/} vagueness requires one to
argue  that the  forms of  language by  which vagueness  is apparently
ascribed  to objects  are  in fact  misleading  idioms, whose  correct
interpretation  does  not involve  genuine  ontological commitment  to
vague objects.
However, contrary to what many proponents of one or other of the two
explanations of vagueness often maintain, accepting that vagueness may be
\emph{de re\/}  does not require one  to deny that  vagueness is often
\emph{de  dicto}.  Indeed,  \citet{Tye90vague-objects}  suggests that
vagueness can be  present both in predicates and  also in objects.  He
argues that  the vagueness  of objects cannot  simply be  explained by
saying that  they are  instances of vague  predicates. 

But the idea of vague objects in the physical world may be hard
to accept. Although at the quantum level of atomic particles we may
conceive of the position of an electron might be vague in a physical
sense, vagueness of  macroscopic physical objects seems a very odd idea.
For example, in consider whether a particular twig is a part of
some pile of twigs, it seems unintuitive to consider the twig pile
as a vague physical object, which may or may not include certain twigs. 
As a palliative to this worry, I propose the existence of \emph{de sensu\/}
vagueness. 

\emph{De sensu\/} vagueness is a kind of indeterminism, in the form of
a multi-faceted structure,  that is located within the
sense, that is in the semantic denotation term. In the
case of names and nominal variables, this means that they can refer
to semantic objects that are indeterminate with regard to any exact
physical entity. Both the model of vagueness proposed in fuzzy logic
\cite{Zadeh65a,Zadeh75a,Goguen69a} and
also the idea of \emph{dot cateogories\/} and \emph{dot objects\/}
proposed in some accounts of co-predication (e.g.\ \cite{arapinis2015plea})
 can be regarded as based on a \emph{de sensu\/} conception of vagueness.





% The  idea  that vagueness  of  objects  is  primarily associated  with
% vagueness of \emph{spatial extension\/} has been endorsed and examined
% by \citet{Tye90vague-objects}, who  gives the following definition of
% a vague (concrete) object:

% A concrete object $o$ is  vague if and only if:
% \begin{enumerate}[label=(\alph*),start=1]
% \item $o$ has borderline spatio-temporal parts;
% \item there is no determinate fact of the matter about whether there
%   are objects that are neither parts, borderline parts, nor non-parts
%   of $o$.
% \end{enumerate}
% 
% Here, I shall not be  particularly concerned with condition (b), which
% is somewhat subtle.  Tye suggests  that (b) is required to account for
% the higher-order  characteristic of  vagueness, that prevents  us from
% making any definite specification  of what are the `borderline' parts
% of an object. Issues  of second-order vagueness are largely orthogonal
% to  the analysis  of vagueness  that I  shall conduct  in  the current
% paper.

% As was mentioned in the  introduction, accepting that vagueness may be
% \emph{de re\/}  does not require one  to deny that  vagueness is often
% \emph{de  dicto}.  Indeed,  \citet{Tye90vague-objects}  suggests that
% vagueness can be  present both in predicates and  also in objects.  He
% argues that  the vagueness  of objects cannot  simply be  explained by
% saying that  they are  instances of vague  predicates.  This  issue is
% central to the  current investigation, and will be  explored in detail
% in subsequent sections of this paper.

% A  somewhat  different picture  of  ontic  vagueness  is suggested  by
% \citet{Barnes10a},   who  proposes   a   metaphysical  interpretation
% characterised in  terms of an intrinsic  indeterminacy regarding which
% possible world is  the actual world.  My main  qualm regarding Barnes'
% account is that what she describes as `ontic vagueness' is more what I
% would call  intrinsic uncertainty (or unknowability).   I shall return
% to  this  issue below,  when  considering  the  ontological status  of
% `things in the world' in (Section~\ref{SEC:whatAreThings}).

\section{Illustrating the Semantics of Predication}


Predication involves a  predicate and a nominal  expression.  Both the
predicate and the nominal can be  given a semantics that allows either
\emph{de dicto\/} vagueness or \emph{de  sensu\/} vagueness or both of
these. \emph{De dicto\/} vagueness is modelled within that part of the
semantics that maps symbolic  expressions (predicates and nominals) to
their referents. If  there is no \emph{de sensu\/}  vagueness then the
referents will be  precise entities, and these will  normally be taken
as  being actual  entities in  the world.   Thus, the  reference of  a
nominal will be a particular  precisely demarcated material entity and
the  reference  of  a  property  (or relation)  predicate  will  be  a
determinate set (or  set of pairs) of material entities.   If there is
\emph{de  sensu\/}  vagueness  then  the  references  of  symbols  are
semantic objects which can be vague  in so far as their correspondence
with precisely demarcated material entities is not fully determinate.

Before specifying  a formal  semantic framework, it  may be  useful to
consider  possible models  of predication  by means  of diagrams.  The
image in  Figure~\ref{FIG:situation+classical}(a)  depicts  an aerial
view of  a hilly region  with rocky crags. As  we see, the  terrain is
irregular  and there  is no  obvious unique  way of  dividing it  into
separate `crag' objects. The name `Arg  Crag' has been given to one of
the rocky outcrops. However, there may be different opinions regarding
exactly which  of outcrop is Arg  Crag. Indeed, some people  might use
the name  to refer  to the  whole of this  rocky area,  whereas others
would consider that it refers to a more specific rock structure.

% \begin{figure}[htb]
% \centerline{
% \includegraphics[width=3in]{figures/the-situation.png}
% }
% \caption{Arg Crag and the surrounding area.}
% \label{FIG:the-situation}
% \end{figure}

In the  standard classical  semantics each  conceptual term  denotes a
fixed set  of entities and  each name must  refer to a  single precise
entity.  Thus, event  before specifying  denotations we  will need  to
divide the craggy  region into specific individual objects,  to make a
set of possible referents:

% \begin{figure}[htb]
% \centerline{
% \includegraphics[width=2in]{figures/classical-predication.png}
% }
% \caption{Standard Classical Semantics.}
% \end{figure}


\begin{figure}[htb]
\centerline{
\parbox{2.7in}{\includegraphics[width=2.6in]{figures/the-situation.png}
%      \mbox{}~~~~~~~~~~~~~~~~~~~~~~~~~~~\textbf{(a)} 
}
~~~~~~~~
\parbox{2.3in}{\includegraphics[width=2.1in]{figures/classical-predication.png}
%     \mbox{}~~~~~~~~~~~~~~~~~~~~~~~~~~~\textbf{(b)} 
}
}
\caption{(a) Arg Crag and surrounding area.~~~~~~~ (b) Classical denotational
  semantics.}
\label{FIG:situation+classical}
\end{figure}


The  best-known approach  to modelling  vague concepts  that has  been
taken in  computer science and  AI is  that of \textit{fuzzy  sets}. A
fuzzy set is one  such at rather than having a  definite true or false
membership condition, there are degrees of membership.
Figure~\ref{FIG:fuzzy+super}(a)
depicts  the standard fuzzy  logic model  of vagueness:  each singular
term  denotes  a single  precise  referent  entity  and each  property
predicate    denotes    a    fuzzy    set   of    precise    entities.
Figure~\ref{FIG:fuzzy+super}(b)  depicts the form of semantics arising
for a
\emph{de  dicto\/}  theory of  vagueness,  where  both properties  and
objects  are  precise but  the  predicate  symbols  and names  of  the
language       that       are       referentially       indeterminate.


\begin{figure}[ht]
\centerline{
\parbox{2.7in}{\includegraphics[width=2.6in]{figures/vague-predication-PsvNsp.pdf}\\
      \mbox{}~~~~~~~~~~~~~~~~~~~~~~~~~~~\textbf{(a)} }
~~~
\parbox{2.3in}{\includegraphics[width=2.1in]{figures/multi-pred-name.png}\\
     \mbox{}~~~~~~~~~~~~~~~~~~~~~~~~~~~\textbf{(b)} }
}
\caption{(a) Fuzzy model of a vague predicate. (b) Multiple denotation
model, such as supervaluation semantics.}
\label{FIG:fuzzy+super}
\end{figure}


One might assume that the blurry concept boundary of the fuzzy logic
model provides a model of predicate denotation that is radically different from
that given by the supervaluationist multi-denotation model. But
it can be argued that this difference is not greatly significant
because we can consider the fuzzy set as essentially equivalent to
a densely nested structure of classical set denotations (one for each
degree of membership value). However, the semantics for evaluating a
predicating expression, $C(\pr{a})$ is significantly different, since
in fuzzy logic the truth value of $C(\pr{a})$ would be the degree of
membership of  object denoted by $\pr{a}$ with respect to the fuzzy
set denoted by $C$; whereas, in the multiple denotation model we
simply get different truth values for different choices and then
(as we shall see in detail below) can determine truth in relation to a
`standpoint' regarding what choices we consider admissible.


A limitation of both the standard fuzzy model and the classical
multiple reference model is that only variability in the terms is
modelled, not variability in the object referred to.  
However, both approaches can be modified to incorporate vague
referents, such as objects with indeterminate physical boundaries.
For instance, objects with fuzzy extensions can be modelled as fuzzy sets of points. 
And within non-fuzzy multiple-reference semantics, one could also
associate a set of different extensions for different precise versions
of an object (or perhaps maximal and minimal extensions, as in the 
`egg-yolk'  representation  of \citet{Cohn96KRvague}).


\begin{figure}[htb]
\centerline{
\includegraphics[width=2.3in]{figures/full-multi.png}
}
\caption{Possible multiplicity of reference when predicates, names and objects
are all indeterminate.}
\label{FIG:full-multi}
\end{figure}

Figure~\ref{FIG:full-multi} 
depicts an extended form of multi-reference semantics (\emph{The Full Multi\/}).
Here we see not only that the predicates and names can have variable
reference, but also there can be multiple possible precise versions of
each reference object. This variability in the objects could
correspond to \emph{de re\/} vagueness, but I prefer to think of it as 
a form of \emph{de sensu\/} vagueness, with the objects being vague
semantic objects (visualised as the small black discs) that correspond to multiple precise physical
objects. 

It is worth noting that Figure~\ref{FIG:full-multi} still represents a
considerable simplification of the potential semantic variability that
might arise. In particular, I have assumed that the global set of vague
objects, together with their associations to precise entities, 
remains fixed, even though the subset associated with predicate
$\pr{C}$ may vary. In other words $\pr{C}$ only varies in how it
\emph{classifies\/} objects, not in how these objects are
\emph{individuated}. 
The VRS semantics presented below is more general. It allows different
senses of sortal predicates to be associated with different ways of
individuating objects (for instance under some interpretations of
`Crag',  all three of the roundish
craggy objects within the innermost circle of the diagram, might be
considered as parts of a single large crag. 





% Figure~\ref{FIG:theory-PmpNmv}  depicts the  semantics of  \LIRAR\ and
% corresponds  to my preferred  account of  the interpretation  of vague
% predicates  and  vague objects.   According  to  this semantics,  both
% predicate  symbols   and  names  are  subject   to  \emph{de  dicto\/}
% vagueness, and the references of  names (and variables) are subject to
% \emph{de sensu\/} vagueness.
% 
% Similarly  to how  LIRAR allows  both referential  (\emph{de dicto\/})
% indeterminacy in  nominal constants and  also \emph{in sensu\/} vagueness
% in  the vague  objects that  are referents  of nominal  constants (and
% variables), it  appears that it would  be be possible  to develop even
% more  elaborate types of  semantics within  which predicates  could be
% both referentially indeterminate and have fuzzy sets of individuals as
% their  possible  referents. However,  it  is  not  clear whether  this
% is necessary  to describe the types of  vagueness found in
% natural language.


% \subsection{Alternative Theories of Vague Reference}
% \label{SEC:alternative-theories}
% 
% \def\figwidthA{2.1in}
% \def\figwidthB{2.6in}
% 
% The semantics  framework of \LIRAR\ can  be regarded as one  case of a
% family of different systems based on the same general idea, but making
% different  choices as  to the  permissible modes  of  indeterminacy of
% predicates and (independently) of singular terms.
% 
% A predication involves a predicate  and a nominal.  Both the predicate
% and the nominal  can be given a semantics  that allows either \emph{de
%   dicto\/}  vagueness  or  \emph{de  sensu\/}  vagueness  or  both  of
% these. \emph{De dicto\/} vagueness is modelled within that part of the
% semantics that maps symbolic  expressions (predicates and nominals) to
% their referents. If  there is no \emph{de sensu\/}  vagueness then the
% referents will be  precise entities, and these will  normally be taken
% as  being actual  entities  in the  world.  Thus, the  reference of  a
% nominal will be a  particular precisely demarcated material entity and
% the  reference  of  a  property  (or relation)  predicate  will  be  a
% determinate set  (or set of pairs)  of material entities.  If there is
% \emph{de  sensu\/}  vagueness  then  the  references  of  symbols  are
% semantic objects which can be  vague in so far as their correspondence
% with precisely demarcated material entities is not fully determinate.
% 
% 
% Rather than present these  as formalised semantic theories, of similar
% form but subtly different to the  one presented above, I think it will
% be  much  easier  to  grasp  the distinctions  if  I  illustrate  them
% diagrammatically.  Figure~\ref{FIG:theory-PspNsp} depicts the standard
% classical semantics in which there is no vagueness. Each singular term
% denotes a  single precise referent entity and  each property predicate
% denotes  a set  of  precise entities.   Figure~\ref{FIG:theory-PsvNsp}
% depicts  the standard fuzzy  logic model  of vagueness:  each singular
% term  denotes  a single  precise  referent  entity  and each  property
% predicate    denotes    a    fuzzy    set   of    precise    entities.
% Figure~\ref{FIG:theory-PsvNsv} depicts  the semantics for  an extended
% fuzzy logic incorporating objects  with vague spatial extensions: each
% singular  term denotes  a  vague object  and  each property  predicate
% denotes a  fuzzy set  of vague objects,  the vague  objects themselves
% could  also   modelled  by  fuzzy  sets  of   points,  although  other
% representations  of the  vague objects  are also  possible  (e.g.\ the
% `egg-yolk'  representation  of \citet{Cohn96KRvague}).\footnote{In  my
%   illustrations I depict an indeterminate property by a blurred region
%   and an indeterminate object by  nested contour lines. This choice is
%   primarily for graphical  purposes: putting blurs on top  of blurs or
%   nested contours  on top of more  nested contours does  not result in
%   very informative diagrams.  My  figures are \emph{not\/} intended to
%   indicate  that the  indeterminacy of  properties is  smooth, whereas
%   indeterminacy  of  objects  is  quantised. Such  characteristics  of
%  indeterminacy are a separate issue.}
  
% \includegraphics[width=2in]{figures/vague-predication-PspNsp.pdf}  
%   
% 
% 
% \vbox{
% \includegraphics[width=2in]{figures/vague-predication-PspNsp.pdf}
% \hbox{(a)}
% }
% 
% 
% \vbox{
% \includegraphics[width=2in]{figures/vague-predication-PsvNsp.pdf}
% \hbox{(b)}
% }
% 
% 
% 
% 
% \begin{figure}[h]
% \centerline{
% \includegraphics[width=\figwidthB]{figures/vague-predication-PsvNsv.pdf}
% }
% \caption{Predicate \pr{C}\ refers determinately to a fuzzy set.
%          Nominal constant \pr{a}\ refers determinately to a vague object.}
% \label{FIG:theory-PsvNsv}
% \end{figure}
% 
% \begin{figure}[h]
% \centerline{ \def\pdfgraphictype{pdf}
% \includegraphics[width=\figwidthA]{figures/vague-predication-PmpNmp.pdf}
% }
% \caption{Predicate \pr{C}\ refers indeterminately to a precise set.
%          Nominal constant \pr{a}\ refers indeterminately to
%          a precise object.}
% \label{FIG:theory-PmpNmp}
% \end{figure}
% 
% \begin{figure}[h]
% \centerline{ 
% \includegraphics[width=\figwidthA]{figures/vague-predication-PmpNmv.pdf}
% }
% \caption{Predicate \pr{C}\ refers indeterminately to a precise set.
%          Nominal constant \pr{a}\ refers indeterminately to
%          a vague object.}
% \label{FIG:theory-PmpNmv}
% \end{figure}






\def\PropStandpointLogic{{\mathbb{S}_0}}

\def\VRSLogic{{\mathbb{V}_1}}



\def\PropConsts{\hbox{$\mathcal{P}$}\xspace}
\def\StandConsts{\hbox{$\mathcal{S}$}\xspace}
\def\PropConst#1{\hbox{$P_{#1}$}\xspace}
\def\StandConst#1{\hbox{$s_{#1}$}\xspace}
\def\Stand{\hbox{$s$}\xspace}
\def\Standp{\hbox{$s'$}\xspace}
\def\pr{\hbox{$\pi$}\xspace}
\def\p#1{\hbox{$\pi_{#1}$}\xspace}
\def\pp{\hbox{$\pi'$}\xspace}
\def\ppp{\hbox{$\pi''$}\xspace}

\def\sp{\hbox{$s'$}\xspace}
\def\st{\hbox{$s$}\xspace}
\def\s#1{\hbox{$s_{#1}$}\xspace}
\def\star{\hbox{$*$}\xspace}


\def\PropConstSet{\{\PropConst{1}\,, \ldots, \PropConst{n} \}}
\def\StandConstSet{\{\StandConst{1}\,, \ldots, \StandConst{m} \}}
\def\PrecSet{\{\ldots, \pr_{i}\,, \ldots \}}

\def\Precs{\hbox{$\Pi$}}
\def\True{\mbf{t}}
\def\False{\mbf{f}}
\def\TruthValSet{\{\True, \False\}}

\def\standb#1{\Box\nolimits_{#1}}
\def\standbs{\standb{s}}
\def\standbsp{\standb{s'}}
\def\standbi#1{\standb{s_{#1}}}
\def\standd#1{\Diamond\nolimits_{#1}}
\def\standds{\standd{s}}
\def\standdsp{\standd{s'}}
\def\standdi#1{\standd{s_{#1}}}
\def\allstandb{\Box\nolimits_{*}}
\def\allstandd{\Diamond\nolimits_{*}}
\def\standindef#1{\mathcal{I}_{#1}\,}
\def\allstandindef{\mathcal{I}_{*}\,}
\def\standdef#1{\mathcal{D}_{#1}\,}
\def\allstanddef{\mathcal{D}_{*}\,}

\def\standbi#1{\square_{s_{#1}}}
\def\standdi#1{\Diamond_{s_{#1}}}

\def\allstandb{\square_{{*}}}


% Models and semantics
\def\modelclass{\mathfrak{M}_{\PropStandpointLogic}}
\def\model{\mathcal{M}}
\def\modelG{\model_\Gamma}

\def\modelequalstuple{\hbox{$\tuple{\Precs, (\accRelation,\preceq), \delta}\,$}}
\def\accRelation{\hbox{$S$}\xspace}
\def\accrelation#1{\hbox{$\s{#1}$}\xspace}
\def\accrelationstar{\hbox{$\star$}\xspace}


\def\deltaP{\delta_{\mathcal{P}}}
\def\deltaK{\delta_{\mathcal{K}}}
\def\deltaQ{\delta_{\mathcal{Q}}}
\def\deltaR{\delta_{\mathcal{R}}}
\def\deltaS{\delta_{\mathcal{S}}}
\def\deltaT{\delta_{\mathcal{T}}}
\def\deltaN{\delta_{\mathcal{N}}}
\def\deltaX{\delta_{\mathcal{X}}}
\def\deltaV{\delta_{\mathcal{V}}}
\def\deltaF{\delta_{\mathcal{F}}}
\def\deltaG{\delta_{\mathcal{G}}}
\def\deltaY{\delta_{\mathcal{Y}}}




\section{Semantic Analysis of Variable Reference}


We now  consider what kind  of semantics  can account for  the general
form       of      variable       denotation      illustrated       in
Figure~\ref{FIG:full-multi}.  \emph{Standpoint Semantics\/} provides a
quite general framework within which polysemy can be modelled in terms
of  the  symbols  of  a   formal  language  having  multiple  possible
denotations.   We shall  start  by specifying  a simple  propositional
standpoint logic and  then elaborate this to  a first-order formalism,
\emph{Variable  Reference  Semantics},  within   which  we  can  model
predication and quantification. But first we explain the basic idea of
standpoint semantics.

Standpoint Semantics is based on a formal structure that models
semantic variability in terms of the following two closely connected
aspects:

\begin{itemize}
\item A \emph{precisification\/} is a precise version of a vague
  language. It is used as an index to assign precise denotations to
  vague terms. The model is based on having a set of precisification,
  each corresponding to a consistent precise interpretation of the
  language.
\item A \emph{standpoint\/} is modelled as a set of
  \emph{precisifications}. Each standpoint corresponds to a range of
  possible precise interpretations that are compatible with a
  particular context of language understanding. It could capture 
  explicit specifications of terminology given by some organisation or implied
  constraints on meanings that arise whenever some vague statement is
  made in conversation (e.g. ``That rock formation is a crag, but this
  is a boulder'').
\end{itemize}


\subsection{Propositional Standpoint Logic}

\subsubsection{Syntax}

The language of  \emph{propositional standpoint logic} 
$\PropStandpointLogic$ is based on a non-empty finite set of propositional variables
\hbox{$\PropConsts = \PropConstSet$}. It extends the usual syntax of
propositional logic by adding  a set of standpoint 
operators $\Sigma = \{ 
\standbi{1}, 
\dots, 
\standbi{n}, 
\allstandb\}$, 
where $\star$ is used to designate the \emph{universal
  standpoint}.\footnote{The language is often augmented by also
  specifying a (partial) order relation over the standpoint operators,
  which indicates that one standpoint may be more specific or more
  general than another. For the purposes of the current paper, we do
  not consider this elaboration the basic system. } 
  So the language of $\PropStandpointLogic$ is the smallest set
  $S$ of formulae such that $\mathcal{P}\subseteq S$ and all
  formulae of the forms 
  $\{\n\phi,\ (\phi\con\psi),\ \square_\sigma \phi\}\subseteq S$ 
  for each $\sigma\in\Sigma$ and every $\phi,\psi \in S$.
One can easily extend the language by defining additional connectives
(e.g.\ $\vee$, $\to$) and the dual operators
($\standdi{1} \dots,
\standdi{n}, 
\Diamond_{\star}$) 
in the usual way.



\subsubsection{Semantics}
In order to characterise the semantics of \emph{standpoint logic\/}
$\PropStandpointLogic$, we
specify a class $\modelclass$ of structures of the form $\tuple{\Pi,S,\delta}$ where:

            \begin{itemize}
            \item $\Precs = \PrecSet$ is a set of precisifications
              (which are analogous to possible worlds),
            \item $S= $ is a set $\{\accrelation{1},...,\accrelation{n},
            \accrelationstar\}$ of subsets of $\Precs$, 
            \item $\delta: \mathcal{P}\imp \wp(\Precs)$ is a function
              mapping each propositional 
variable $p\in\mathcal{P}$ to the set $\delta(p)\subseteq \Precs$ of precisifications
            at which it is true. (Here,  $\wp(\Precs)$ denotes the
            powerset of $\Precs$.)
%\alert{correct this. OR} $\delta$ is the interpretation function mapping from natural numbers to sets of possible worlds such that for each number $n$, $P_n$ is the subset of $\Precs$, $\delta(\mathcal{P}_n)\subseteq\Precs$, where the propositional variable $\mathcal{P}_n$ is true (as in \cite{Chellas1980ModalIntroduction}) 
            \end{itemize}


The most distinctive elements of  the model are the $\accrelation{i}$,
which model  the notion  of standpoint via  a set  of precisifications
that are \emph{admissible\/} for that standpoint. Thus, if $\pr
\in \s{i}$ then all propositions that are unequivocally true according
to standpoint $\s{i}$ are true at precisification $\pr$.

		               
For a model structure $\mathcal{M}\in \modelclass$, we write $(\model,
\pr)  \models  \phi$  to  mean  that  formula  $\phi$  is  true  at  a
precisification   $\pr\in\Precs$  in   $\mathcal{M}$.   For  a   model
$\mathcal{M} = \tuple{\Pi,S,\delta}$, this relationship is defined by:

\begin{itemize}
    \item $(\model, \pr) \models P$\ \ if and only if\ \ $\pr \in \delta(P)$,
    \item $(\model, \pr) \models \n \alpha $ \ if and only if\  $(\model, \pr) \nvDash \alpha$,
	            \item $(\model, \pr) \models \alpha \con \beta$ 
	            \ if and only if 
	            $(\model, \pr) \models \alpha$ and $(\model, \pr) \models \beta$,
	            \item $(\model, \pr) \models \standbi{i} \alpha$
                      \ if and only if
               $(\model, \pp) \models \alpha$ for all 
                      $\pp \in \accrelation{i}$. 
	            \item $(\model, \pr) \models \allstandb \alpha$
                      \ if and only if
               $(\model, \pp) \models \alpha$ for all $\pp\in\Pi$. 
\end{itemize}

		    
A  formula   $\phi$  is  \emph{valid\/}   if  it  is  true   at  every
precisification of every model in $\modelclass$. In this case we write
$\models_{\mathbb{S}_0} \phi$.

\vspace{1ex}

The logic $\PropStandpointLogic$ enables one to formalise the content of statements such
as. ``Arg is definitely either a crag or a boulder. This map labels it
a crag, but I would say it could be called either, although a boulder is
different from a crag.'' With {\sf Ba} and {\sf Ca} meaning respectively
`Arg is a boulder' and `Arg is a crag', one could write:

\def\pr#1{\mathsf{#1}}
$$
\Box_{\star}(\pr{B}\pr{a} \dis \pr{C}\pr{a}) 
\ \con \
\Box_{\textit{map}}\pr{C}\pr{a}
\ \con \
\Diamond_{\textit{me}}\pr{B}\pr{a} 
\con 
\Diamond_{\textit{me}}\pr{C}\pr{a} 
\con
\Box_{\textit{me}}\n(\pr{B}\pr{a} \con \pr{C}\pr{a}) 
$$



\subsection{Variable Reference Logic}
\label{SEC:VRL}

We now generalise the standpoint semantics framework to 
define a first-order variable reference logic $\VRSLogic$
that can represent predication and quantification.\footnote{In this
presentation, we omit specifying the semantics for propositional
connectives and standpoint
operators and just give the semantics for predication and
quantification in terms of truth conditions at a particular
precisification in a given model. A more comprehensive semantics
could be given by incorporating, with slight modification, the
relevant specifications from the propositional semantics.}


\subsubsection{Syntax}

The language of $\VRSLogic$ is built from a vocabulary
$\mathcal{V} =
\tuple{\mathcal{K},\mathcal{P},\mathcal{Q},\mathcal{N},\mathcal{X}}$,
comprising the following symbols:
\begin{itemize}[itemsep=0ex,label=$\bullet$]
   \item $\mathcal{K} = \{ \ldots, \mathsf{K}_i, \ldots \}$ is a set of count-noun symbols (sortals),
   \item $\mathcal{P} = \{ \ldots, \mathsf{P}_i, \ldots \}$ is a
     set of individual property predicates,
   \item $\mathcal{Q} = \{ \ldots, \mathsf{Q}_i, \ldots \}$
    is a set of precise entity property predicates, \hfill
    (e.g.\ exact spatial properties)
   \item $\mathcal{N} = \{ \ldots, \mathsf{n}_i, \ldots \}$
    is a set of proper name symbols.
   \item $\mathcal{X} = \{ \ldots, x_i, \ldots \}$
    is a set of nominal variable symbols.
\end{itemize}

The symbols of $\mathcal{K}$, $\mathcal{P}$ and $\mathcal{Q}$ can all
be applied as predicates, with the sortal symbols of  $\mathcal{K}$
also being used to specify a range of quantification.
Symbols of both $\mathcal{N}$ and $\mathcal{X}$ can both occur as
arguments of predicates, although the variable symbols of
$\mathcal{X}$ are only meaningful in the context of quantification.

The set $S$ of formulae of  $\VRSLogic$ is the smallest set such that:

\begin{enumerate}[label=$\bullet$,itemsep=0ex]
\item 
$\{ \alpha(\tau) \ | \ 
 \alpha\in (\mathcal{K}\!\cup\!\mathcal{P}\!\cup\!\mathcal{Q}),
 \tau\in (\mathcal{N}\!\cup\!\mathcal{X})\} \subseteq S$
\hfill (contains all atomic predication formulae)
\item  
$\{\n\phi,\ (\phi\con\psi),\ \Box_{s_i} \phi,\ \Box_{\star}\phi \} \subseteq S$\ \ for every $\phi,\psi\in S$ 
\hfill (closed under connectives)
\item
$(\A \pr{K}\!:\!x)[\phi] \in S$ for every $\pr{K}\in\mathcal{K}$ every
  $x\in\mathcal{X}$ and every $\phi \in S$ 
\hfill (includes quantified formulae)
\end{enumerate}


% \def\pr#1{\mathsf{#1}}
% \begin{enumerate}[itemsep=0ex,label=$\bullet$]
% \item $\pr{K}(\tau)$ \ \ \ sortal predication
% \item $\pr{P}(\tau)$ \ \ \ non-sortal individual property predication
% \item $\pr{Q}(\tau)$  \ \ \ precise property predication
% % \item $\pr{R}(\omega_1,\omega_2)$ \hfill individual relational predication
% % \item $\pr{S}(\mu_1,\mu_2)$ \hfill material relational predication
% % \item $(\omega_1 = \omega_2)$     \hfill object identity
% % \item $(\rho_1 = \rho_2)$         \hfill spatial region identity
% % \item $(\tau_1 = \tau_2)$         \hfill material property value identity
% % \item $\pr{Part}(\omega_1 = \omega_2)$ \hfill object parthood
% % \item $\pr{Part}(\rho_1 = \rho_2)$   \hfill region parthood
% \end{enumerate}


\subsubsection{Semantics}

The semantics for variable reference logic $\VRSLogic$ will be
based on structures
$\tuple{ E, \Pi, \mathcal{V}, \delta }$
where:
\begin{enumerate}[label=$\bullet$,itemsep=0ex]
\item $E$ is the set of precise entities.
\item $\Pi$ is the set of precisifications.
\item $\mathcal{V} = \tuple{ \mathcal{K}, \mathcal{P}, \mathcal{Q},
  \mathcal{N}, \mathcal{X} }$ 
   is the non-logical vocabulary, as specified above,
\item $\delta = \tuple{  
         \delta_{\mathcal{K}},
         \delta_{\mathcal{P}},
         \delta_{\mathcal{Q}},
         \delta_{\mathcal{N}},
 \delta_{\mathcal{X}} }$ is a denotation function that can be
  considered as divided into components specifying the denotations for
  each type of non-logical symbol (see below).
\end{enumerate}

To simplify the explanation of the semantics, I first
define the semantic representation of a \emph{indefinite individual}.
(Here, and in the following, $B^A$ denotes the set of all functions from domain set $A$
into the range set $B$):
\begin{itemize}
\item $I = E^\Pi$ is the set of (indefinite) individuals, each of
  which   is a mapping from the set of precisificaiton indices $\Pi$ to the
  set of precise entities. 
\end{itemize}
For each individual $i\in I$
  and each precisification $\pi\in\Pi$, the value of $i(\pi)$ will be
  a precise version of individual $i$ according to precisification $\pi$.

\vspace{1ex}

\noindent The denotation functions for all the non-logical
vocabulary of the language as follows:
\begin{itemize}
\item $\delta_{\mathcal{K}} : \mathcal{K} \to  \wp(I)^\Pi$ \ \  is a
  function mapping each sortal concept (count noun) in
  $\mathcal{K}$ to a function from precisifications to sets of indefinite individuals.
\end{itemize}
On the basis of $\delta_{\mathcal{K}}$ we define
     $I_{\pi} =  \bigcup \{ \delta_{\mathcal{K}}(\mathsf{K})(\pi) \ |
  \ \mathsf{K} \in \mathcal{K}\}$,
the set of all individuals of any sort according to precisification $\pi$. 
We can now define:
\begin{itemize}
\item $\delta_{\mathcal{P}} : \mathcal{P} \to  \wp(I)^\Pi$, \ 
 such that,  for all $\mathsf{P} \in \mathcal{P}$\ 
   we must have $\delta_{\mathcal{P}}(\mathsf{P})(\pi) \subseteq I_\pi$.
\item $\delta_{\mathcal{Q}} : \mathcal{Q} \to  \wp(E)$ \ \  
    \ \  (each precise predicate is associated with a set of precise entities)

\item $\delta_{\mathcal{N}} : \mathcal{N} \to  \wp(I)^\Pi$, \  
 subject to the condition that,  for all $\mathsf{n} \in \mathcal{N}$
   we must have $\delta_{\mathcal{N}}(\mathsf{n})(\pi) \in
   I_\pi$.

\item $\delta_{\mathcal{X}} : \mathcal{X} \to  \wp(I)$, 
  \ \ \   (but the semantically relevant denotations of variables are
  determined by sortals occurring in quantifiers)  
\end{itemize}


\subsubsection{Interpretation of Reference and Predication}

For a model $\mathcal{M} =\tuple{ E, \Pi, \mathcal{V}, \delta }$ and
precisification $\pi\in \Pi$, the truth conditions for atomic
predication formulae are as follows:
\begin{itemize}
    \item $(\model, \pi) \models \pr{K}(\pr{n})$\ \ if and only if\ \ 
             $(\deltaN(\pr{n}))(\pi) \in (\deltaK(\pr{K}))(\pi)$

    \item $(\model, \pi) \models \pr{P}(\pr{n})$\ \ if and only if\ \ 
             $(\deltaN(\pr{n}))(\pi) \in (\deltaP(\pr{P}))(\pi)$

    \item $(\model, \pi) \models \pr{Q}(\pr{n})$\ \ if and only if\ \ 
              $((\deltaN(\pr{n}))(\pi))(\pi) \in \deltaQ(\pr{Q})$

    \item $(\model, \pi) \models \pr{K}(x)$\ \ if and only if\ \ 
             $\deltaX(x) \in (\deltaK(\pr{K}))(\pi)$

    \item $(\model, \pi) \models \pr{P}(x)$\ \ if and only if\ \ 
             $\deltaX(x) \in (\deltaP(\pr{P}))(\pi)$

    \item $(\model, \pi) \models \pr{Q}(x)$\ \ if and only if\ \ 
              $(\deltaX(x))(\pi) \in \deltaQ(\pr{Q})$
\end{itemize}

To  make  sense  these  specifications  you  need  to  be  aware  that
evaluation  of a  symbol  may  require zero,  one,  or  two levels  of
de-referencing in  relation to  the precisification index  $\pi$.  You
should  first note  that the  $\pr{K}$ and  $\pr{P}$ predications  are
semantically equivalent.   When applied to  a name constant,  {\sf n},
both the  constant and the predicate  get evaluated with respect  to a
precisification, so that the name  denotes a particular individual and
the predicate denotes a set of such individuals.  When the argument is
a variable rather than a  name constant, the variable directly denotes
an  individual  without   any  need  for  evaluation   relative  to  a
precisification.   In  the  case  of  (exact)  $\pr{Q}$  predications,
individuals   need   to  be   further   evaluated   relative  to   the
precisification  in order  to obtain  a precise  entity, which  can be
tested  for  membership  of  the   precise  set  denoted  by  property
$\pr{Q}$. So  although $\pr{Q}$ predicates are  not themselves subject
to  variation in  relation  to  $\pi$ the  impose  an  extra level  of
variability in the interpretation their argument symbol.

It may seem curious that the same precisification index $\pi$ is used
both for mapping names (and predicates) to individuals (and sets of individuals), and
also for mapping from individuals to precise entities. Thus the
individual denoted by a name {\sf n} in precisification $\pi$ 
is $(\deltaN(\pr{n}))(\pi)$ and according to $\pi$ it also refers to
the precise entity $((\deltaN(\pr{n}))(\pi))(\pi)$. This slightly
simplifies the specification and does not
appear to place any constraint on the semantics.

\subsubsection{Interpretation of Quantification}

To facilitate specification of
the semantics for quantification, I
define a meta-level operation $\mathcal{M}^{(x_i\Rightarrow \xi)}$
on interpretation structures that enables us to replace the value of a
variable with a new value.
For
$\mathcal{M} =\tuple{ E, \Pi, \mathcal{V}, \delta }$, 
with  
$\mathcal{V} = \tuple{ \mathcal{K}, \mathcal{P}, \mathcal{Q},  \mathcal{N}, \mathcal{X} }$, 
$\delta = \tuple{  
         \delta_{\mathcal{K}},
         \delta_{\mathcal{P}},
         \delta_{\mathcal{Q}},
         \delta_{\mathcal{N}},
 \delta_{\mathcal{X}} }$,
and $\xi\in E^\Pi$
let
$\mathcal{M}^{(x_i\Rightarrow  \xi)}$ be the structure 
$\mathcal{M}' =\tuple{ E, \Pi, \mathcal{V}, \delta' }$,
where 
$\delta'  = \tuple{  
         \delta_{\mathcal{K}},
         \delta_{\mathcal{P}},
         \delta_{\mathcal{Q}},
         \delta_{\mathcal{N}},
 \delta'_{\mathcal{X}} }$
and $\delta'_{\mathcal{X}}(x_j) = \delta_{\mathcal{X}}(x_j)$
for every $x_j\neq x_i$ and $\delta'_{\mathcal{X}}(x_i) = \xi$. 

Finally we can specify the interpretation of a quantified formula:

\begin{itemize}
\item
$(\mathcal{M}, \pi)\  \models\  (\A\,\pr{K}\!:\! x)[\phi(x)] 
       \hbox{~~~~if and only if~~~~} 
   (\mathcal{M}^{(x_i\Rightarrow  \xi)}, \pi)\  \models\  \phi(x)
\hbox{~~for all}\ \xi \in \deltaK(\pr{K})(\pi)$
\item
$(\mathcal{M}, \pi)\  \models\  (\E\,\pr{K}\!:\! x)[\phi(x)] 
       \hbox{~~~~if and only if~~~~} 
   (\mathcal{M}^{(x_i\Rightarrow  \xi)}, \pi)\  \models\  \phi(x)
\hbox{~~for some}\ \xi \in \deltaK(\pr{K})(\pi)$
\end{itemize}

This is much the same as how one would specify quantification in a
classical sorted logic. The universally quantified formula is true
just in case its immediate sub-formula is true for all possible values
of the variable, taken from the range of the sortal predicate.

\subsubsection{What Can $\VRSLogic$ Express?}

So was  the result  worth all  the work  of defining  that complicated
semantics?   Does  it  help   us  understand  and  represent  semantic
variability   and   its   effect   on   reference,   predication   and
quantification.  Yes, I  think so.  Although the  final definitions of
the quantifiers  seem simple, one  needs to consider  that significant
work has been done by the denotation functions for the different kinds
of symbol  and the semantics  given above  for the different  cases of
predication.  Their effect is to allow quantification to operate at an
intermediate level  in the  interpretation of semantic  variability of
reference.  The  \emph{individuation\/} of potential  referents occurs
prior to quantification  by establishing individuals in  relation to a
given interpretation  of sortal predicates. But  these individuals can
still  be indeterminate  in that  they  may correspond  to many  exact
entities.

Consider the statement ``There is definitely a mountain in Equador,
that some say is on the equator and others say it is not''. This might
be represented as:
$$
\Box_{\star}(\E\, \pr{Mountain}\!:\!x)
[\ \pr{InEquador}(x) \con 
 \Diamond_{\star}[\pr{OnEquator}(x) \con  \Diamond_{\star}[\n\pr{OnEquator}(x)]\ ]
$$

I believe that this kind of statement cannot be represented without
using a semantics that can account for both \emph{de dicto\/} and
\emph{de re\/} forms of vagueness. Its truth conditions require that
there is something that is definitely a mountain and definitely in
Equador but whose extent is ill defined such that it could reasonably 
be said either that it does or does not lie on the equator.


% =========
% 
% $$
% \mathcal{M} = \tuple{ \mathcal{V}, D,
%   0, V,  \sigma, \Pi, \delta} \ ,
% $$  
% with $\delta=$ $\langle\deltaK, \deltaP,$
%   $\deltaR,     \deltaN,    \deltaF,     \deltaX,     \deltaY\rangle$,    let
% $\mathcal{M}^{(x_i\Rightarrow  \xi)}$ be the  interpretation structure
% %%exactly  like  $\mathcal{M}$   except  that  $\mathcal{M}'  =  
% $\langle
%   \mathcal{V},    D,   0,    V,   \sigma,$    $\Pi,    \delta'\rangle$,   with
% $\delta'=\tuple{\deltaK, \deltaP, \deltaR, \deltaN, \deltaF, \deltaX',
%   \deltaY}$,  where $\deltaX'$ is  defined by  $\deltaX'(x_i)=\xi$ and
% $\deltaX'(x_j)=\deltaX'(x_j)$  for every  $x_j$ in  $\mathcal{X}$ such
% that $x_j\neq x_i$.
% 
% Thus, $\mathcal{M}^{(x_i\Rightarrow \xi)}$ is exactly like $\mathcal{M}$,
% except that $\mathcal{M}^{(x_i\Rightarrow \xi)}$ assigns the value
% $\xi$ to the varable $x_i$. (The structures may be identical if 
% $\mathcal{M}$ also assigns $\xi$ to  $x_i$.)
% 
% I now stipulate that:
% \begin{equation*}
% \begin{split}
% \mathcal{M}, \pi\ & \Vdash\  (\A\,\pr{K}: x)[\phi(x)] 
%        \hbox{~~~iff~~~} \\
%   & \mathcal{M}^{(x_i\Rightarrow  \xi)}, \pi\  \Vdash\  \phi(x)
% \hbox{~~for all}\ \xi \in \deltaK(\pr{K})(\pi) \\
% % & \mathcal{M} \stackrel{x\to \xi}{\Longrightarrow} \mathcal{M}'
% %   \hbox{~for some~} \xi \in \deltaK(\pr{K})(\pi) \ .
% \end{split}
% \end{equation*}
% 
% And similarly, for the existential quantifier:
% \begin{equation*}
% \begin{split}
% \mathcal{M}, \pi\ & \Vdash\  (\E\,\pr{K}: x)[\phi(x)] 
%        \hbox{~~~iff~~~} \\
%   & \mathcal{M}^{(x_i\Rightarrow  \xi)}, \pi\  \Vdash\  \phi(x)
% \hbox{~~for some}\ \xi \in \deltaK(\pr{K})(\pi) \\
% %   & \mathcal{M}', \pi\  \Vdash\  \phi(x)
% % \hbox{~~for some model}\ \mathcal{M}' \hbox{~such that~}\\
% %  & \mathcal{M} \stackrel{x\to \xi}{\Longrightarrow} \mathcal{M}'
% %    \hbox{~for some~} \xi \in \deltaK(\pr{K})(\pi) \ .
% \end{split}
% \end{equation*}

% $$
% (\E\,\pr{K}:x)[\phi(x)] \equivdef \n(\A\,\pr{K}:x)[\n\phi(x)] 
% $$


% \subsection{Deep Ambiguity in Sortal Concepts}
% 
% A \emph{sortal\/} concept is one that carries with it criteria 
% for individuating and counting entities.
% Hence one might expect that sortals should at least be unambiguous
% when it comes to the fundamental criteria for being an instance
% or at least the general ontological category of the objects that
% can instantiate them.
% However this is not the case.
% 
% Mary loves cats. Whenever she encounters a cat she wants to stroke it. 
% In her art class she often paints cats. She even has cats on the wallpaper of her bedroom.
% 
% Thomas Pynchon has written nine books and I've got two of them on my bookshelf.
% 
% This book is heavy but informative.



\def\pr#1{\hbox{$\mathsf{#1}$}}

\section{Co-Predication and Deep Polysemy of Sortal Concepts}

I now turn to another issue involving polysemy and reference, that I
admit not having properly considered during the whole time I was
constructing the VRS logic described above: the issue of
co-predication
\cite{asher2011lexical,arapinis2015plea,gotham2017composing,liebesman2017copredication,viebahn2020copredication}.
When I first became aware that people were studying 
this phenomenon as an issue in its own right, rather than just being
a particular case of polysemy, I was somewhat surprised. And even
after preliminary consideration, I assumed that it could be handled
without special difficulty within the double level model
of semantic indeterminacy provided by VRS. However, once I had got
more deeply
acquainted with the problem I came to realise that it does require
special attention. This section will be a largely informal
discussion of the topic.


\subsection{The Problem of Co-Predication}

A \emph{sortal\/} concept is one that carries with it criteria 
for individuating and counting entities.
Hence one might expect that sortals should at least be unambiguous
when it comes to the fundamental criteria for being an instance
or at least the general ontological category of the objects that
can instantiate them.
However this is not the case.
Consider the sentence ``There is a book by Olaf Stapledon on my bookshelf.'' With the simplification of treating 
being on my bookshelf as a simple predicate we would get the following `naive' classical representation:
\begin{equation*}
\begin{split}
\E x  [ \pr{Book}(x) \con \pr{By}(x,\pr{OS}) \con  \pr{OnMyBookShelf}(x) ]
\end{split}
\end{equation*}
A problem with this representation is that the predicate \pr{Book} appears to be polysemous between the sense of being an informational artifact and being a physical object. And, moreover, whereas the authorship predicate, \pr{By}, applies to the informational sense, the predicate \pr{OnMyBookShelf} applies to the physical sense. 
It is this application to a single referent of two predicates 
that seem to describe very different kinds of object that is called
co-predication. The issue is not just that \pr{Book} has two senses but that the predications seem to imply the existence of an object that is an instance of both senses of \pr{Book}.

One might expect that this problem could be avoided by adopting the view that books are a type of object that has both an information and a physical aspect and that different types of predicate that can be applied to books must be interpreted with respect to the aspect appropriate to the type of predicate (authorship applying to the informational aspect and physical properties to the physical aspect of book). But, unfortunately, the idea of multi-aspect objects can only account for very simple examples. Consider, the sentence: 
``There are two books by Olaf Stapledon on my bookshelf.''

\begin{equation*}
\begin{split}
\E x \E y [x\neq y & \con \pr{Book}(x) \con \pr{Book}(y) \\
                   & \con \pr{By}(x,\pr{OS}) \con \pr{By}(y,\pr{OS}) \\
                   & \con \pr{OnMyBookShelf}(x) \con \pr{OnMyBookShelf}(y) ]
\end{split}
\end{equation*}

The problem is  that determining how many books by  Olaf Stapledon are
on my  self depends  upon whether  I count  in terms  of informational
artifacts or  physical volumes. I  might have  two copies of  the same
book, or  two book titles  contained within  the same volume  (or some
more  complex combination  of volumes  and contents).   Thus, a  claim
regarding the  number of books can  only have definite meaning  once I
choose what  kind of book object  I wish to count.  But accepting this
leads  to a  recapitulation  of  the original  problem.  Once I  choose
between informational and physical books,  I am no longer dealing with
entities that can support both the informational property of the books
content originating  from a  particular author  and also  the physical
property of being a physical object located on a particular shelf.


Before considering some proposals made in the literature regarding how
one  might account  for co-predication,  let  us first  note that  the
VRS  theory of  predicates  and   vague  objects  given  above  
(Section~\ref{SEC:VRL})  fails   to  provide   a  straightforward
explanation of typical co-predication examples.
That  semantics  both  allows  vagueness  of  sortal  predicates  that
categorise and individuate objects over which we may quantify and also
allows  these   objects  to  have   properties  that  are   not  fully
determinate, such as a mountain, whose boundary is unclear.
So maybe the complicated VRS semantics could make sense of the
following formulation:
$$
(\exists\,\pr{Book}\!:\!x)[\pr{ByOS}(x) \wedge \pr{OnMyBookShelf}(x)]
$$
But for this to work, we would need to assume that the polysemy of
book is within the semantic object denoted by $x$ so that the two
predicates can be evaluated with respect to different aspects of some
multi-faceted book object that has both physical and informational
aspects. 
However, the problem of individuation and counting still remains.
Although VRS allows that {\sf Book} can have different senses
both in terms of individuation and in terms of exact entities, 
it is based on the assumption that any ambiguity in individuation
criteria is resolved prior to determining the set of individuals
over which  the quantifier $(\exists\,\pr{Book}\!:\!x)$ will range.
Hence, although we can have both indeterminate counting criteria
and indeterminate individuals, we cannot have indeterminate individuals whose
precise correlates satisfy different counting criteria.
In the case of vague of geographic features, for example, one might
say that `individuation must precede demarcation'.

\subsection{Towards a Solution}

Many approaches, some very clever and most rather complex, have been
proposed for accounting for co-predication. I will not consider these
in the current paper except to mention that some have proposed that
co-predication involves mechanism for \emph{coercion\/} or
\emph{inheritance\/}
between different categories of entity that can be referred to by 
polysemous nouns that exhibit co-predication phenomena 
\cite{asher2011lexical,liebesman2017copredication},
some have proposed special
kinds of compound ontological categories
(e.g.\ \cite{arapinis2015plea}) 
and some have proposed complex semantics of individuation (e.g.\ 
\cite{gotham2017composing}). None of the proposals I have encountered
so far seems completely satisfactory to me.

My  view is that  different  individuation  conditions must  be
associated with different precisifications of  the count noun. I don't
think  we can  individuate  objects  unless we  have restricted the
interpretation of the term to the extent that it enables individuation.
The VRS approach does allow different modes of individuation to be
associated with different senses of a sortal concept, which could
account for the radically different ontological types associated with 
certain count nouns such as `book'. But if this is the case, we still
need to account for co-predication examples where it seems that 
individual objects exhibit multiple ontologically diverse aspects.
Such possibilities would need to be specified in terms of type
conversions that can occur due to context, and are often unambiguous
due to corresponding entities of a different type being uniquely
determined in many cases (e.g.\ in many particular situations 
a physical book instance uniquely determines and informational book
and a reference to an informational book determines a unique physical book). 


% However,  these  do not  necessarily  correspond  to senses  that  are
% associated with entities of a single ontological category.
% 
% Gotham's mechanism is quite ingenious.
% I would consider Gotham's composition of physical and information
% individuation criteria to be a specific and not typical sense of book.

\section{Conclusions and Further Work}

The paper has explored the issue of multiple possible references of linguistic terms, that may arise due to vagueness of terms or differences in opinions on how they should be interpreted, and how such variability effects the semantics of reference, predication and quantification, as conceived within a denotational approach to semantics.
I have proposed the framework of \emph{variable reference semantics} to interpret a logical language in a way that can account for both \emph{de dicto\/} vagueness in predicates and also \emph{de re}, or, as I would prefer to call it \emph{de sensu\/} variability in the `objects' that are referred to. 

The system presented is intended more as a proof of concept than a workable formal language. The semantics is rather complex but when formulating representations within the object language of the logic $\VRSLogic$ much of this complexity is hidden under the bonnet.
However, the utility of the system remains to be demonstrated beyond a few relatively simple examples. The main direction for further work would be to consider a much wider range of examples and evaluate the strengths and limitations of the proposed formalism. As for formal logic in general, I do not really envisage the system being used in its full blown form, but rather some aspects of the language and semantics might be used in a restricted form to support various kinds of application, such as, for example, querying of information systems.

The other direction in which I would like to extend the work is with further consideration of issues such as co-predication, which would test the limitations of the system in dealing with semantic phenomena related to semantic variability.


\skipover{
================================
\vspace{1cm}


An ontologist might say such a representation is plain wrong or that the formula under its standard interpretation does not adequately capture the semantics of the assertion.

\cite{viebahn2020copredication}


I first read \emph{First and Last Men\/} by Olaf Stapledon when I was a student. I read it a again last year but I had lost my original copy so had to buy it again. 

However, it seems that in many cases this kind of \emph{copredication\/} does not cause any difficulty in conveying information.

It certainly seems natural that we can mix the physical and informational interpretations of `book' in many situations. One can pick up a book and say `This book is by Olaf Stapledon.' 

Co-predication occurs when one polysemous nominal expression has simultaneous
predications selecting for two different meanings or senses. Anaphoric binding of different
senses of a polysemous noun occurs when a pronominal expression takes a sense that is
different from the sense attributed to its antecedent noun. 

\subsection{The Problem of Co-Predication}



\subsection{Theoretical Models of Co-Predication}

There are two main views:
\begin{itemize}
\item A word such as `book' is lexically ambiguous. That is the word has two meanings. Asher
\item A word such as `book' categorises objects that are semantically composite. Vieu Gotham
\end{itemize}

\href{https://e1.pcloud.link/publink/show?code=XZeMWRZgwAFlLdng0XPXpII9umGVhTRJyKX}{Viebahn 2020 Copredication}  \cite{viebahn2020copredication}

\href{https://e1.pcloud.link/publink/show?code=XZeMWRZgwAFlLdng0XPXpII9umGVhTRJyKX}{Gotham Thesis}

\cite{gotham2017composing}



\subsection{Mutliple-Individuation Senses}

The problems in counting 

Gotham \cite{gotham2017composing} uses the theory of pluralities of Link \cite{link2002logical}.

Different senses have different individuation criteria giving rise to different counting principles. This difference can be located within the equality relation associated with a particular mode of individuation. 


According to Gotham the individuation criteria appropriate for counting objects in a given context are induced by the predicates in which they occur. 
Predicates that apply to an informational sense of book will give rise to counting in terms of informational objects and those applying to physical objects will induce counting in terms of physical volumes. And in the case of co-predication involving both informational and physical properties are `composed' by taking the union of the equality relations for each mode.
In the case of books, this means that, when one counts `informative' `heavy' books, one should count entities that are distinct both in terms of informational content and physical constitution.


co-predicated 

There is a subsequent criticism in
\cite{liebesman2019copredication}.

\cite{ortega2019polysemy}

\subsubsection{Dot Objects}

Distributional analysis \cite{jezek2014distributional}

Mereological dot objects \cite{arapinis2015plea},


Collins
\cite{collins2017copredication}
\cite{collins2021diversity}


\subsection{Contextual Coercion of Referent}

This is the idea that a references to categorically ambiguous objects (a dot object, such as book) can be automatically converted by the context in which they occur to reference to an entity of the category appropriate for that context.

\subsection{My Solution??}

Co-occurrence of exemplars.
If two things always occur together it is natural that they are referred to by one word.

This is fine as long as they always occur together (ie have always aligned individuation criteria) but can be problmatic when the criteria are not always aligned. (As in the case of books).
However, even in cases that are not strictly aligned there can be very strong alignment is a wide range of contexts. eg One will typically be considering a particular physical book corresponding to a particular informational artifact or several physical books that in most cases will be 1:1 aligned with information artifacts. Hence, counting the physical and informational object will be aligned.

Maybe a collective object can have different plurality numbers with respect to different aspects.

But what about quantification as a higher order operator:
eg Every student had read two of the recommended books.

Two of the recommended books had been read by every student.

$$
(\E_2 \pr{Book}: x)[\pr{Read}(s,x)]
$$

Quantification seems ok in terms of standpoints.
On the standpoint account we take as a starting standpoint, one that is not committed as to whether books should be counted in terms of physical volumes or in terms of informational artifacts. 
In many cases a sentence will come out true for both of these interpretations so will be unequivocal. But in some cases the count could be correct according to one interpretation but incorrect according to another.

But what about co-predication? Well that would need to be done in terms of aspects of an entity.
The problem comes when there is not a one-to-one mapping.

They banned the book and ordered it to be burned.

For a book in the information sense to be burned it suggests that copies of it should be burned. 


Eg. ``This is  not a book!''. Cannot be considered as false under the interpretation that book must be an informational artifact.

\subsubsection{Solving Copredication with Standpoins}

The bigger problem for me seems to be the copredication rather than the quantification. 

We cannot find global precisifications that satisfy two predicates, because the senses are disjoint.
We must have some kind of compound object.

The compound object must have mappings to both the physical and informational.

My proposed solution is that count nouns that exhibit co-predication phenomena have multiple senses of individuation that are used to pick out objects from a network of property bearing entities. These entities are of two or more distinct ontological types (e.g.\ physical and informational) but tightly linked by relationships linking different ontological categories. A paradigm case would be books, where we have physical volumes and informational artifacts. 

For simplicity I first consider a very simple structuring of the linked entity types. Let us assume that the relationship between physical volumes and informational books is such that every physical volume corresponds to exactly one informational artifact, but each informational artifact can correspond to any number of physical volumes. 



In contrast to some other proposals I neither propose that we should 

My view is  



Can have an ove-specified joint meaning. One where we assume that there is a unique pairing between physical and informational books.
I think this would do it. It would show that certain contexts require standpoints in which there is a 1-1 correspondence.

Could there be two compound senses but differing in counting criteria?


\subsection{Prolific Ontological Heterogeneity of the Term `Meal'}

In much of the research on co-predication, the example of `book' has been taken as a paradigm case. This is certainly a good example to consider, since `book' has two clearly distinct modes of individuation (physical volumes \textit{vs.} information artifacts) as well as some interesting complication, such as collected works, multi-volume publications and variant editions. However, the fact that there are only two clearly different individuation modes (albeit with some complications) means that the co-predication possibilities are somewhat limited compared to other examples with much more diversity in possible modes of individuation.

I suggest that the issue of multiple individuation criteria is better illustrated by the term `meal', which is much more prolific in the number of ways one might count its instances. The word meal is vague in a huge number of ways. There are many considerations relating to `borderlne' issues, such as the distinction between a few mouthfuls and a meal or whether there could be a meal where nobody actually ate anything (e.g. the dining hall was evacuated due to a fire alarm). But we are now interested only in polysemy relating to fundamental ontological type giving rise to different modes of individuation and counting. I suggest that the following six individuation modes can be distinguished.:  

\begin{enumerate}[label=(\Alph*)]
\item A type of eating event, usually differentiated by time of day it is eaten, but also associated with a range of typical foods: 
   \begin{itemize}
    %\item ``Breakfast is my favourite meal.'', 
    \item ``Half board accommodation includes two meals. You can choose either breakfast and lunch or breakfast and dinner. Full board includes four meals: breakfast, lunch, afternoon tea and dinner.''
   \end{itemize}
\item An eating event occurence which can be solitary but often involves multiple people participating in the same meal.
  \begin{itemize}
    \item ``The conference programme included two meals: a reception buffet and a formal dinner''
  \end{itemize}
\item An individual eating event:
  \begin{itemize}
    \item ``One pizza and one salad is enough food for three meals.''
    \item ``We ate together at the bistro. John loved his meal and we both liked the food, but I didn't enjoy my meal as I kept thinking about the money I had lost.''
 \end{itemize}
   Here, we could further differentiate senses where we are thinking of the actual food from senses where we are thinking about other aspects of the experience. What is essential to this mode is that the `meal' count will be the same as the number of people involved.
    % We could further differentiate between a sense where we refer to the individual's experience of the food (``John did not enjoy his meal because he does not like anchovies'')  and a sense where we refer to other aspects of the event (``John didn't enjoy his meal because he kept thinking about the exam he had to take the next day.''). However, this sense distinction does not seem to affect how one would individuate and count meals.
\item A physical food portion. That is, a quantity of food prepared for (and usually served to) an individual person during a particular time interval: 
  \begin{itemize}
    \item ``The students ordered 8 meals between them --- 5 pizzas and 3 omelettes. 2 of the students just ordered a beer.''
    \item 
    ``The refectory prepares over 500 meals each day. Usually fewer than 20 go to waste.''
 \end{itemize}
 \item A physical food ensemble intended for a group of people:
    \begin{itemize}
      \item  Three meals had been laid out. One on each of the three tables. Each of the meals was for four people.  
    \end{itemize}
 \item A particular food type or collection of food types often eaten together:
   \begin{itemize}
     \item ``Pancakes (with blueberries) is one of my favourite meals.'' 
     \item ``The menu lists five set meals including two vegetarian meals''
   \end{itemize}
  \item Complex eating event types. One can potentially specify and enumerate a wide variety complex eating event types. Such meal types are listed in certain kinds of menu:
   \begin{itemize}
      \item ``The cruise offers three special meals, which you can book as many times as you wish:
          oysters and champagne in your cabin,
          tea and cake for two on the poop deck,
          fish dinner at the captain's table.
     \end{itemize}
     Meals individuated by mode (F) have a similar 
     ontological status to those of
     mode (A) but are more specialised and are typically combined with food specifications akin to mode (F); and they support a counting mode that is distinct from either (A) or (F).
\end{enumerate}

Figure~(\ref{FIG:meal-ontology}) shows the connections between meal senses (A)--(F) in terms of categories of designated entities and corresponding referential phrases in a typical example, that might be described by the sentence ``John and Mary ate pancakes for breakfast together.''
We see that despite the possible senses spanning many ontological categories associated with different ways in which `meals' can be counted, in a typical situation the associations between entities of the different categories is relatively straightforward. The eating event (involving both participants) can be associated with a type of meal (breakfast) and with a physical ensemble of food items (all the pancakes and accompanying edible accoutrements), which can be  described as a particular meal type. We also have the possibility of dividing the joint eating event into tow individual events, each corresponding to a food portion (some part of the ensemble). The situation would be a little more complex if the two had eaten different foods. But we can see that in many situations, identifying a referent in terms of an entity of one ontological category would uniquely determine a referent of another associated category.

\begin{figure}
\centerline{
\includegraphics[width=4in]{figures/meal-ontology.png}
}
\caption{\centerline{Some senses of `meal' with different modes of individuation.}}
\label{FIG:meal-ontology}
\end{figure}

The meal with my new colleges was really entertaining and 
delicious too. 



\subsection{An Enhanced Model}

My suggestion is that different individuation conditions must be associated with different precisifications of the count noun. I don't think we can individuate objects unless we have settled upon an interpretation of the term that enables individuation.



However, these do not necessarily correspond to senses that are associated with entities of a single ontological category. 

Gotham's mechanism is quite ingenious.
I would consider Gotham's composition of physical and information individuation criteria to be a specific and not typical sense of book.
}


%%
%% The acknowledgments section is defined using the "acknowledgments" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
% \begin{acknowledgments}
%   Thanks to the developers of ACM consolidated LaTeX styles
%   \url{https://github.com/borisveytsman/acmart} and to the developers
%   of Elsevier updated \LaTeX{} templates
%   \url{https://www.ctan.org/tex-archive/macros/latex/contrib/els-cas-templates}.  
% \end{acknowledgments}

%%
%% Define the bibliography file to be used
\bibliography{huge,newbrandon,local}

% %%
% %% If your work has an appendix, this is the place to put it.
% \appendix

% \section{Online Resources}

% The sources for the ceur-art style are available via
% \begin{itemize}
% \item \href{https://github.com/yamadharma/ceurart}{GitHub},
% % \item \href{https://www.overleaf.com/project/5e76702c4acae70001d3bc87}{Overleaf},
% \item
%   \href{https://www.overleaf.com/latex/templates/template-for-submissions-to-ceur-workshop-proceedings-ceur-ws-dot-org/pkfscdkgkhcq}{Overleaf
%     template}.
% \end{itemize}


